Quickest change detection with unknown parameters: Constant complexity and near optimality

We consider the quickest change detection problem where both the parameters of pre- and post- change distributions are unknown, which prevents the use of classical simple hypothesis testing. Without additional assumptions, optimal solutions are not tractable as they rely on some minimax and robust variant of the objective. As a consequence, change points might be detected too late for practical applications (in economics, health care or maintenance for instance). Available constant complexity techniques typically solve a relaxed version of the problem, deeply relying on very specific probability distributions and/or some very precise additional knowledge. We consider a totally different approach that leverages the theoretical asymptotic properties of optimal solutions to derive a new scalable approximate algorithm with near optimal performance that runs~in~$\mathcal{O}(1)$, adapted to even more complex Markovian settings.

==> Src/rebuttal.tex <==
We thank the reviewers for their constructive feedback and quality reviews. 
We start by answering a common concern for all the reviewers then we address each of them regarding the remaining remarks. We  want to highlight that our contribution targets specifically the computational complexity vs detection delay trade-off. To the extent of our knowledge, we display state of the art performances for change detection algorithms that run in $\mathcal{O}(1)$ (c.f.\ Section \ref{sec:related_works}). 

\textbf{Near optimality guarantees:}
    Our theoretical results (Lemma 1-3) combined with the annealing/penalisation procedures justify that our algorithm efficiently approximates $L_t^*$. 
    We believe that this in itself is an asymptotic performance guarantee: In fact, evaluating the performance boils down to evaluating the detection delay w.r.t.\ the Shiryaev stopping time $\mathds{E}[|\boldsymbol\nu - \boldsymbol\nu_\alpha^S |]$. This quantity is proportional to the estimation error $\mathds{E}[ |S_n^{\theta_n^0, \theta_n^1} - S_n^{\theta_0^*, \theta_1^*}| ]$, which in turn is proportional to $ \mathds{E}[|L_t-L_t^*|] $. 
    However deriving explicitly this relationship is not only cumbersome (integrating over all possible stopping time scenarios), but also requires additional assumptions over the convergence rate of Equation \ref{shiryaev_asymp}. In principle, for carefully selected hyper-parameters, our algorithm will inherit the same asymptotic properties of Equation \ref{shiryaev_asymp} modulo the approximation errors.
    %For these reasons, we chose to defend our algorithm with theoretically grounded insights and experimental results (over a wide variety of settings) rather than additional assumptions over this speed of convergence. 

\textbf{Reviewer 2:} 
    Equation 5 quantifies (asymptotically) the delay of optimal detection rules, this is why it provides insights about the true change point. Intuitively, our idea is to iteratively assume we reached the Shiryaev stopping time, learn the change point distribution under this assumption and use it to evaluate the parameters. Then we update $S_n$ to check whether we were wrong or not and move on to the next observation. Compared to the GLR, we are not evaluating all possible change points but only those that would make the current observation a probable stopping time. 
    
\textbf{Reviewer 4:} 
    We respectfully disagree with the reviewer. Our main claim (as stated in the abstract, the introduction and in Section \ref{sec:related_works}) is that we achieve the best performance for algorithms with constant complexity (running in $\mathcal{O}(1)$). The GLR procedure (discussed in Section \ref{sec:related_works} along with recent sota change detection techniques) is costly despite the interesting properties it exhibits. \\
    We agree that the recent works of Tartakovsky et al. contain important results regarding optimal change detection rules in general. However, they do not subsume our contribution. Our paper is the first  to exploit asymptotic behaviour of optimal procedure to produce fast and reliable detections. Stronger results might help improve the procedure, but Equation \ref{shiryaev_asymp} is sufficient to produce the desired goal. We also point out our disagreement with the novelty assessment of the reviewer. \\
    Regarding the remaining remarks: \textbf{1-} Using the Shiryaev-Robert statistic (a particular case of the Shiryaev statistic) is possible, and produces similar results to the ones reported in the experiments. \textbf{2-} We agree that the bulk of the paper does not address multi-task problems. However that setting is what motivated the need for reliable \textbf{and} fast detection rules. This is why we included it in the title. Nonetheless, we are considering changing it to avoid confusion. 
    
\textbf{Reviewer 5:} 
    \textit{Lemma 1}: We assume that the family is properly parametrised (c.f.\ Section \ref{sec:QCDP}). Moreover, even when it is not the case, it doesn't affect the performances empirically (c.f.\ the last paragraph of Appendix \ref{A:copy-cat}).\\ \textit{Baselines}:   GLR is an optimality baseline as it provably provides the best possible evaluation in parametric settings, thus reaching comparable performances to it is sufficient. As for approximate solutions, we used the adaptive approach in the synthetic data case, and we also used a MLE over recent observations in the RL settings. In both cases, we out-performed both methods. Moving average rules are not suited for this setting as  data is not i.i.d. We also point out that optimal solutions (GLR, BOCPD, etc) slightly outperformed TWR in the RL settings. However, we only compared  to algorithms with constant complexity (in $\mathcal{O}(1)$) as it is the scope of the paper.\\ \textit{Penalisation}: the constant c helps control the trade-off between low PFA and low ADD: in figure 6, adding this penalisation increased the ADD, but we can see in Figure 5, that adding it reduces $L_t$ before the change point (thus reducing the PFA). {\color{red} More on this in the Figure bellow.}\\
    \textit{Sigmoid}: this approximation entails from the choice of a Logistic distribution to approximate the posterior distribution of the change point ($|\nu_\alpha^S=n$). This choice is itself motivated in (L195). $d$ is defined in L129 using the prior distribution over $\boldsymbol\lambda$.\\ \textit{L092}: $\boldsymbol\lambda$ is a random variable generated from the prior.\\ \textit{L167}: for practical reasons, $t_2$~is assumed finite, see (L163).
    
\textbf{Reviewer 6:} 
    Figures 2-3 evaluate the regretted ADD for various cutting thresholds $B_\alpha$ (c.f. Appendix \ref{appendix:QCD} for the mapping between $B_\alpha$ and $\alpha$). The three algorithms are evaluated for the same threshold as we vary it. {\color{red}We provide bellow an evaluation of both ADD and PFA in similar conditions.}
    
\newpage
{\color{red} A mettre directement sur le site !}
\textbf{For the meta-reviewer:}
    We would like to point out our strong disagreement with Reviewer\#4. Despite being an expert of the domain, he/she missed the point of the paper (Notice that the other reviewers did not struggle with highlighting the scalability contribution). Reviewer \#4 also falsely accused us of duplicating existing work and suggested that we are very far behind current state of the art. This is not backed by any evidence in his/her review. While interesting, none of the cited resources proposed a similar/better algorithm that runs in $\mathcal{O}(1)$. Most of them actually confirm the optimality of the GLR approach (runs in $\mathcal{O}(n^2)$). The GLR is the baseline we used in our experiments to justify near-optimality empirically.
    We also highlight that all the other reviewers agreed that this is a worthy contribution if not more.
